Dynamic and Transparent Analysis of Commodity Production Systems

We propose a framework that provides a programming interface to perform complex dynamic system-level analyses of deployed production systems. By leveraging hardware support for virtualization available nowadays on all commodity machines, our framework is completely transparent to the system under analysis and it guarantees isolation of the analysis tools running on its top. Thus, the internals of the kernel of the running system needs not to be modified and the whole platform runs unaware of the framework. Moreover, errors in the analysis tools do not affect the running system and the framework. This is accomplished by installing a minimalistic virtual machine monitor and migrating the system, as it runs, into a virtual machine. In order to demonstrate the potentials of our framework we developed an interactive kernel debugger, nicknamed HyperDbg. HyperDbg can be used to debug any critical kernel component, and even to single step the execution of exception and interrupt handlers.

==> vtx.tex <==
\section{Hardware Assisted Virtualization}
\label{sec:vtx}

Virtualization, once only used in specialized systems, is now becoming broadly
available in simpler system. Latest CPUs, both Intel and AMD, include hardware
support for virtualization. In this Section, we focus on Intel Virtualization
Technology, that our framework leverages to allow deep inspection of a system's
kernel.

In a non-virtualized system, the operating system controls all hardware
resources. On the other hand, a virtualized system includes a new layer, the
\emph{Virtual-Machine Monitor} (VMM), that rules accesses to the physical
resources of the machine. The VMM allows to run multiple operating systems,
namely ``guests'', \emph{concurrently} on the same machine presenting to each
of them different virtual platform interfaces, i.e. ``virtual
machines''~\cite{neiger06}.

Intel Virtualization Technology, whom in the following we will refer to as
VT-x, introduces two new CPU operating modes: \emph{VMX root operation} and
\emph{VMX non-root operation}. The first is used by the VMM while the latter is
used by the VMs and is controlled by the VMM. In software-only virtualization,
since the VMM runs at the most privileged level, the guest OS has to be run at
a different (higher) level. Many techniques have been proposed and used to
overcome this limitation but all of them introduce great complexity and many
problems. VT-x allows to bypass this limitation since both root and non-root
mode support four privilege levels (rings), actually allowing a guest to run at
its intended privilege level. A transition from root mode to non-root mode is
called \emph{VM Entry} while the inverse transition is called \emph{VM
  Exit}. To manage these switches, a data structure (VMCS) is used. The VMCS is
divided in two parts: the \emph{guest-state area} and the \emph{host-state
  area}. During each switch, the CPU takes care of saving its state in the
appropriate area and loading the correct state from the other area. That is to
say, whenever a VM Entry is performed, the processor state is saved in the host
area and loaded from the guest area and vice versa, during a VM Exit, the
processor state is saved in the guest area and loaded from the host area.

\subsection{VM Exits}
% While in root operation mode there are no substantial behavior changes in
% respect to an IA-32 architecture without VT-x support, when in non-root mode,
% processor operations undergo some significant changes.
VM Exits are triggered in response to particular instructions and events
(interrupts and exceptions) that happen in non-root mode~\cite{intel:3B}. Some
instructions trigger an exit unconditionally, like \texttt{cpuid}, while others
cause an exit only depending on VMM settings or other conditions. For example,
an instruction that accesses one of the \texttt{CR} CPU registers causes a VM
exit only if certain conditions set by the VMM hold. Events that can trigger an
exit include exceptions and interrupts. VM Exits store information, such the
instruction which caused them, in the VMCS, so that the VMM can handle them
correctly.

To avoid a VMM to become greatly complex, it is possible to set a number of
fields in the VMCS, namely the \emph{VM-Execution Control Fields}, that allow a
fine-grained specification of which events should trigger VM Exits. This
feature has a key role for the performance of a VMM. Consider, for example,
timer-based interrupts. These interrupts are generated at a very fast rate and,
if not needed by the VMM, would cause an unbearable overhead due to the high
number of consequent VM Exits. By settings appropriate flags and values of
bitmaps included in the VM-Execution Control Field, the VMM can selectively
specify which events are of interest and discard others. The VMCS includes
bitmaps to mask exceptions and I/O operations. Our framework uses these two
bitmaps, as we will describe in detail in the following Sections, to grant
transparency to the guest OS and to offer debugging features like breakpoints
and single stepping. \FIXME{Another use of these bitmaps regards I/O bitmaps,
  that contain one entry for each port of the I/O space. Our framework uses
  these bitmaps to trap \texttt{IN} instructions that access the keyboard I/O
  port, in order to transparently gather pressed keys in root mode.}\JOY{Non so
  se va bene questo esempio o se \`e meglio lasciarlo solo nella sezione
  apposita}

VM Exit are usually ``fault-like'', meaning that the instruction that is
triggering a VM Exit is not executed before the switch from non-root to root
mode~\cite{intel:3B}. After the switch, the VMM must then deal with the cause
that triggered the exit. The VMM can decide to emulate the faulty instruction
or event or to allow its execution, returning control to the guest. The first
option will be discussed case per case in the following of the paper, while we
discuss the second one in Section~\ref{entry}.

\subsection{VM Entries}\label{entry}
As mentioned above, VM Entries are used to return control to the guest and to
load processor state from the guest-state area of the VMCS. Furthermore, an
entry can \emph{inject} an event (exception or interrupt) into the
guest~\cite{neiger06}. VM Entries deliver an injected event only after all
components of the guest-state have been loaded. By doing so, events are
injected in the guest context~\cite{intel:3B}. The injection is performed by
invoking the handler contained in the guest Interrupt Descriptor Table. This
feature greatly reduce the complexity of a VMM, since it allows to ignore
non-relevant events that should otherwise be emulated by the VMM. VM Entry
event injection has to be dealt with carefully. For example, to guarantee a
correct functioning of a guest operating system, some software interrupts
should be delivered only under certain conditions. Consider the case of
software interrupt~\#3, commonly used by debuggers to set breakpoints. Our
framework, as we will illustrate in the following of the paper, allows to set
software breakpoints from root mode and consequently intercepts every
interrupt~\#3 to handle them. To guarantee guest OS consistency, only interrupts
that have been caused purposely by the guest (e.g. if the guest is running an
user-space debugger) must be injected, while interrupts caused by breakpoints
set by our framework must be handled in root mode and then discarded.


% \FIXME{Da cambiare -- preso da KEmuFuzzer}

% Our oracle leverages Intel technology for hardware assisted virtualization,
% namely VT-x~\cite{neiger06}. By using hardware-assisted virtualization, we can
% observe the execution of the test-case on the physical CPU without losing the
% ability to interrupt the execution and to inspect the state of the CPU at any
% time, even when it enters invalid states. Intel VT-x technology transforms
% Intel x86 (and x86-64) ISA into something much more virtualization-friendly
% than a ISA that meets Popek and Goldberg minimal requirement for efficient
% virtualization. Besides not having any critical instruction, VT-x allows to
% configure dynamically which instructions must trap and in which conditions.
% Furthermore, VT-x includes a new mode of operation (VMX), that essentially adds
% new higher privilege rings for running the virtual machine monitor, that is,
% the software component the host uses to manage guests. The introduction of
% these new rings allows a clear separation between host and guests, which is not
% invasive for guests. Indeed, system code of the guest is executed natively on
% the CPU in system-mode. Nevertheless, the host still needs to assume the
% control of the guest in certain situations (e.g., to redirect I/O operations to
% devices emulated via software). Clearly, the challenge is to develop a
% minimalistic software component for the host, that is sufficiently
% sophisticated to execute a test-case and to hold complete control of the
% execution, but that is also simple enough to be verifiable.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% ispell-local-dictionary: "american"
%%% End: 

